Solving Continual Offline Reinforcement Learning with Decision Transformer

Continuous offline reinforcement learning (CORL) combines continuous and offline reinforcement learning, enabling agents to learn multiple tasks from static datasets without forgetting prior tasks. However, CORL faces challenges in balancing stability and plasticity. Existing methods, employing Actor-Critic structures and experience replay (ER), suffer from distribution shifts, low efficiency, and weak knowledge-sharing. We aim to investigate whether Decision Transformer (DT), another offline RL paradigm, can serve as a more suitable offline continuous learner to address these issues. We first compare AC-based offline algorithms with DT in the CORL framework. DT offers advantages in learning efficiency, distribution shift mitigation, and zero-shot generalization but exacerbates the forgetting problem during supervised parameter updates. We introduce multi-head DT (MH-DT) and low-rank adaptation DT (LoRA-DT) to mitigate DT's forgetting problem. MH-DT stores task-specific knowledge using multiple heads, facilitating knowledge sharing with common components. It employs distillation and selective rehearsal to enhance current task learning when a replay buffer is available. In buffer-unavailable scenarios, LoRA-DT merges less influential weights and fine-tunes DT's decisive MLP layer to adapt to the current task. Extensive experiments on MoJuCo and Meta-World benchmarks demonstrate that our methods outperform SOTA CORL baselines and showcase enhanced learning capabilities and superior memory efficiency.

==> section/sec1_intro.tex <==

\section{Introduction}
Unlike machines, humans possess a remarkable capacity for continuous learning and adaptation throughout their entire lifespan. This unique capability is referred to as continuous learning(CL). Much previous work has focused on enabling reinforcement learning algorithms to have the ability to continuously learn, which means quickly learning new tasks in sequential interactions with online environments, and avoiding forgetting previous tasks~\citep{rolnick_ahuja_schwarz_lillicrap_wayne_2018,isele_cosgun_2022,zenke_poole_ganguli_2017}. However, in some scenarios, collecting new data and interacting with the environment may bring high costs or serious consequences, so it is precious to use existing data for efficient, safe, and transferable learning. \citet{Gai_Wang_He_2023} proposed continuous offline reinforcement learning (CORL), a novel paradigm that combines continuous learning and offline reinforcement learning, which aims to enable agents to learn multiple tasks from static offline datasets and quickly adapt to new unknown tasks. A primary and long-standing challenge in CORL is the plasticity-stability trade-off \citep{Khetarpal_Riemer_Rish_Precup_2022}: the RL policy on the one hand needs to retain the knowledge and avoid forgetting tasks in history (stability) while on the other hand can be quickly adapted to new tasks (plasticity). \ls{too long. We should simplify this part.}

Existing methods mainly combine the offline algorithm
based on actor-critic structure and continual learning methods \citep{Gai_Wang_He_2023} in which rehearsal-based methods ~\citep{lopez-paz_ranzato_2017,chaudhry_ranzato_rohrbach_elhoseiny_2018} are the most popular. These methods suffer a lot such as multiple distribution shifts, low learning efficiency and weak knowledge-sharing capabilities. 
There are three types of distribution shifts. The first is the distribution shift between the behaviour policy and the learning policy, which is unavoidable in all offline algorithms using Actor-Critic structures and inevitably leads to the over-estimation problem of the out-of-distribution (OOD) data; the second is the distribution shift between the offline data of each task, which also causes catastrophic forgetting; the last one is the possible distribution shift between the learned policy and the saved replay buffer when using the experience replay method, which will lead to performance declines in previous tasks during the rehearsal process. 
The learning efficiency is low because the AC-based offline algorithm needs to learn the Q function and the policy at the same time which then causes the knowledge of the learned policy cannot be well distilled into the current agent in limited training steps.
As for knowledge-sharing capability, although the Q function has been proven to be relevant in related tasks ~\citep{Niekerk_James_Earle_Rosman_2019}, these methods only add behavioural clones to the action network, which is unexplainable because the objective of the actor is to maximize the Q value, thus leading to weak knowledge-sharing capabilities. \ls{too long. We should simplify this part. This paragraph mainly focuses on the drawbacks and challenges of CORL. The motivation of this paper}



To solve the above problems, we first rethink the precess of  CORL by comparing an AC-based offline RL algorithm with Decision Transformer (DT) \citep{Chen_Lu_Rajeswaran_Lee_Grover_Laskin_Abbeel_Srinivas_Mordatch_2021}, another offline RL paradigm in the CORL setting. The results demonstrate several advantages of DT, such as high learning efficiency, bypassing the distribution shift problem, and better zero-shot generalization ability. However, the forgetting issue of DT in CORL setting which updates all parameters during continuous learning is more serious. This is because DT is trained using supervised learning and is more sensitive to distribution shifts between time-evolving  datasets. 


In order to retain the advantages of DT and solve the more serious problem of catastrophic forgetting, we propose multi-head DT (MH-DT) and low-rank adaptation DT (LoRA-DT). MH-DT uses multiple heads to store task-specific knowledge and share knowledge with common parts, to avoid the catastrophic forgetting problem caused by all parameters being changed when the dataset distribution shift occurs. Besides, using the structural characteristics of the transformer and the feature that DT will benefit from training on close tasks we propose an additional distillation objective and selective rehearsal module to improve the learning effect of the current task.
To solve the CORL problem when the replay buffer is not allowed – for example, in real-world scenarios where data privacy matters\citep{Shokri_Shmatikov_2015}, inspired by \citet{Lawson_Qureshi_2023} that explored the similarities and differences of each module in the DT structure under multi-task situations, we proposed LoRA-DT that merges weights that have
little impact for knowledge sharing and fine-tunes the decisive MLP layer in DT blocks with LoRA to adapt to the current task. This method also avoids substantial performance deterioration with a smaller buffer size \citep{Cha_Lee_Shin_2021}.

Extensive experiments on MuJoCo \citep{EmanuelTodorov2012MuJoCoAP} and Meta-World \citep{yu2020meta} benchmarks demonstrate that our methods outperform SOTA baselines in all CORL metrics. Our DT-based methods also show other advantages. For example, the learning effect of MH-DT is more robust when the number of review tasks increases. Saving the updated $\mA\mB$ matrix to avoid forgetting previous tasks in LoRA-DT has also proven to be a more memory-efficient method compared with saving replay buffers.
% In summary, this paper rethinks the CORL problem with decision transformer and points out the advantages of using DT to solve CORL and the problems that need to be solved. To leverage the benefits and solve the problem of catastrophic forgetting, we propose two methods, MH-DT and LORA-DT for the scenarios where the replay buffer is available and unavailable respectively. 
The main contributions of this paper can be summarized as four folds:
\begin{itemize}
    \item We propose that compared to the offline reinforcement learning method using Actor-Critic structure, the method using DT as the basic model is more suitable for solving the CORL problem and points out the advantages of DT problems that need to be solved by rethinking the CORL process with decision transformer. To the best of our knowledge, we are the first to propose using DT as an infrastructure in CORL setting. 
    \item When the replay buffer is available, we propose the MH-DT model to solve the problem of catastrophic forgetting and avoid the problem of low learning efficiency when the number of tasks increases by distillation and selective rehearsal.
    \item When the buffer is unavailable, we proposed LoRA-DT, which uses weights merging and low-rank adaptation to avoid catastrophic forgetting and save memory by saving the fine-tuned $\mA\mB$ matrix instead of the buffer.
    \item We experimentally demonstrate that our methods outperform prior CORL methods, perform better in scenarios with a large number of tasks, and are more memory-efficient.
\end{itemize}


% Reinforcement learning (RL) has shown great success in solving sequential decision problems such as board games
% ~\citep{JulianSchrittwieser2019MasteringAG}, computer games ~\citep{LukaszKaiser2019ModelBasedRL}, and robotics ~\citep{MarvinZhang2018SOLARDS,AnushaNagabandi2018LearningTA}. However, a notable limitation of existing approaches is their tendency to focus on training agents to excel in narrow, well-defined tasks. Unlike machines, humans possess a remarkable capacity for continuous learning and adaptation throughout their entire lifespan. This unique capability is referred to as continuous learning(CL). Much previous work has focused on enabling reinforcement learning algorithms to have the ability to continuously learn, which means quickly learning new tasks in sequential interactions with online environments, and avoiding forgetting previous tasks~\citep{rolnick_ahuja_schwarz_lillicrap_wayne_2018,isele_cosgun_2022,zenke_poole_ganguli_2017}. Moreover, online learning sequential tasks is not always feasible due to the temporal and spatial constraints of the environment and the agent's on-board consideration itself.

% Offline RL learns from pre-collected datasets instead of directly interacting with the environment ~\citep{Fujimoto_Meger_Precup_2018}. By leveraging pre-collected datasets, offline RL methods avoid costly interactions and thus enhance learning efficiency and safety, has been recognized as a method that is more practical in real-world scenarios. Recently, \citet{Gai_Wang_He_2023} proposed a new setting named continual offline reinforcement learning (CORL), which integrates offline RL and continual learning, letting agents learn sequentially through offline datasets.

% The major challenge of continual learning is how to alleviate the catastrophic forgetting ~\citep{McCloskey_Cohen_1989} issue on previous tasks when learning new tasks. Under ideal conditions, the RL policy on the one hand needs to retain and reuse the knowledge shared across different tasks in history (stability) while on the other hand can be quickly adapted to new tasks without interference from previous tasks (plasticity). There are three types of continual learning methods, including regularization-based methods \citep{zenke_poole_ganguli_2017,kirkpatrick2017overcoming}, modular methods \citep{Fernando_Banarse_Blundell_Zwols_Ha_Rusu_Pritzel_Wierstra_2017,Mallya_Lazebnik_2018}, and rehearsal-based methods ~\citep{lopez-paz_ranzato_2017,chaudhry_ranzato_rohrbach_elhoseiny_2018}. OER \citep{Gai_Wang_He_2023} argues that ER \citep{rolnick_ahuja_schwarz_lillicrap_wayne_2018}, a widely-used rehearsal-based method, is the most suitable method for CORL problems and proposed a method that combines shared modules and experience replay to achieve a trade-off between stability and plasticity.

% The CORL problem is very difficult to solve because it is affected by three kinds of distribution shifts. The first is the distribution shift between the behaviour policy and the learning policy, which is unavoidable in all offline algorithms using Actor-Critic structures and inevitably leads to the over-estimation problem of the out-of-distribution (OOD) data; the second is the distribution shift between the offline data of each task, which also causes catastrophic forgetting; the last one is the possible distribution shift between the learned policy and the saved replay buffer when using the experience replay method, which will lead to poor performance in previous tasks during the rehearsal process.

% As a basic module for large models in other fields such as CV and NLP\citep{brown2020language,ramesh2021zero}, transformer\citep{vaswani2017attention} exhibits strong long-sequence memory capabilities and generalization capabilities. \citet{Chen_Lu_Rajeswaran_Lee_Grover_Laskin_Abbeel_Srinivas_Mordatch_2021} presented Decision Transformer, an architecture that casts the problem of RL as conditional sequence modelling. In this paper, we propose that compared to the offline reinforcement learning method using Actor-Critic structure, the method using DT as the basic model is more suitable for solving the CORL problem, see details in Sec.\ref{chp:rethink}. The decision transformer is more aware of tasks, trains faster, and will benefit from training on similar tasks. However, there are some problems in directly applying decision transformer to CORL problems, such as forgetting which is more serious \ls{not clear. Why?}.  



% \ls{the challenges of continual offline RL should be reorganized. }
% \ls{summarize the challenges of continual offline RL as several-fold. and expanse these challenges. e.g.: common challenges of CORL; the challenges of CORL with DT. }
% \ls{be careful! The mentioned challenges could be solved by our methods.}


% In order to retain the advantages of the decison transformer and solve the more serious problem of catastrophic forgetting, we proposed MH-DT, a method that combines the shared structure method and the review method. Selectively reviewing the experience of previous tasks and updating the head of each task and the common part at the same time, not only solves the problem of catastrophic forgetting but also solves the problem of the previous CORL method that when the number of tasks increases, the agent can't learn a well-performed policy for later tasks because there are too many tasks that need to be reviewed.

% In addition, although the ER methods have proven to work best\citep{Gai_Wang_He_2023}, they suffer from substantial performance deterioration with smaller buffer size \citep{Cha_Lee_Shin_2021} and become ineffective when a rehearsal buffer is not allowed – for example, in real-world scenarios where data privacy matters\citep{Shokri_Shmatikov_2015}. In order to solve the CORL problem when the replay buffer is unavailable, we combined the characteristics of transformer and proposed a more space-saving low-rank adaptation(LoRA) method to solve the catastrophic forgetting problem. \citet{Lawson_Qureshi_2023} explored the similarities and differences of each module in the DT structure under multi-task situations. Inspired by this article, we proposed to use LoRA to fine-tune the MLP layer in each block of the transformer for each task, and save the $\mA\mB$ matrix to avoid forgetting previous tasks.







% In summary, this paper rethinks the CORL problem with decision transformer. The advantages of using DT to solve CORL and the problems that need to be solved are pointed out. This article proposes two methods, MH-DT and LORA-DT for the scenarios where the replay buffer is available and unavailable respectively. The main contributions of this paper are four folds:
% \ls{the contribution parts should be polished.}

% \begin{itemize}
%     \item To the best of our knowledge, we are the first to propose using DT as an infrastructure to solve the CORL problem. \ls{the first is not a contribution. The problem we solve  is the contribution. We should first say:  we propose XXXX . To the best of knowledge we are the first xxxx. }
%     \item When the replay buffer is available, we propose the MH-DT model to solve the problem of catastrophic forgetting and avoid the problem of low learning efficiency when the number of tasks increases by selective rehearsal.
%     \item When the buffer is unavailable, we proposed LoRA-DT, which uses low-rank adaptation to avoid catastrophic forgetting and save memory by saving the fine-tuned $\mA\mB$ matrix instead of the buffer.
%     \item We experimentally demonstrate on a variety of benchmarks that our methods outperform prior CORL methods and perform better in scenarios with a large number of tasks and save memory.
% \end{itemize}

